Efficient Sampling of Temporal Networks with Preserved Causality Structure

In this paper, we extend the classical Color Refinement algorithm for static networks to temporal (undirected and directed) networks. This enables us to design an algorithm to sample synthetic networks that preserves the $d$-hop neighborhood structure of a given temporal network. The higher $d$ is chosen, the better the temporal neighborhood structure of the original network is preserved. Specifically, we provide efficient algorithms that preserve time-respecting ("causal") paths in the networks up to length $d$, and scale to real-world network sizes. We validate our approach theoretically (for Degree and Katz centrality) and experimentally (for edge persistence, causal triangles, and burstiness). An experimental comparison shows that our method retains these key temporal characteristics more effectively than existing randomization methods.

==> applications.tex <==
The datesets are:  gre (grenoble), ren (rennes), bel (belfast) and kuo (kuopio) and social contact traces from {\href{sociopatterns.org}{sociopatterns.org}} namely: prim (primaryschool), hs11 (HighSchool2011), hs12 (HighSchool2012), hp (Hospital Ward), ht (HyperText) and wp (Workplace). All datasets are available publicly.

\begin{table}[h!]
    \centering
      \resizebox{\textwidth}{!}{  
    \begin{tabular}{l|cccccc}
    \hline  
dataset & nodes & events & edges & agg\_edges & $\#$ possible rewirings \\ \hline
gre & $1547$ & $1300$ & $113112$ & $3680$ &\\
ren & $1407$ & $10825$ & $107384$ & $3718$ & \\
bel & $1917$ & $1132$ & $120951$ & $6440$  &\\
kuo & $549$ & $1211$ & $30545$ & $1952$  &\\
prim & $242$ & $3100$ & $125773$ & $16634$ & \\
hs11 & $126$ & $5609$ & $28539$ & $3418$  &\\
hs12 & $180$ & $11273$ & $45047$ & $4440$ &\\
hp & $75$ & $9453$ & $32424$ & $2278$  &\\
ht & $113$ & $5246$ & $20818$ & $4392$ & \\
wp & $92$ & $7104$ & $9827$ & $1510$  &\\
    \end{tabular}
    }
    \caption{Statistics for the datasets. From left to right  number of nodes (nodes), number of times (events), number of temporal edges (edges), number of edges in the static representation of $G$.}
    \label{tab:gen_stat}
\end{table}

List of possible rewirings of wp for $d=1$ 

